Dissecting AI Trading: Behavioral Finance and Market Bubbles

We study how AI agents form expectations and trade in experimental asset markets. Using a simulated open-call auction populated by autonomous Large Language Model (LLM) agents, we document three main findings. First, AI agents exhibit classic behavioral patterns: a pronounced disposition effect and recency-weighted extrapolative beliefs. Second, these individual-level patterns aggregate into equilibrium dynamics that replicate classic experimental findings (Smith et al., 1988), including the predictive power of excess demand for future prices and the positive relationship between disagreement and trading volume. Third, by analyzing the agents' reasoning text through a twenty-mechanism scoring framework, we show that targeted prompt interventions causally amplify or suppress specific behavioral mechanisms, significantly altering the magnitude of market bubbles.

==> Tables/Table_bidoffer_pricechange_half.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular*}{1.0\hsize}{@{\hskip\tabcolsep\extracolsep\fill}l*{4}{cc}}
\toprule
                    &\multicolumn{4}{c}{Price Changes (t to t+1)} \\
                    \cline{2-5}
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}\\
\midrule
Bid-Offer x Second Half Dummy&     -0.0164\sym{***}&     -0.0242\sym{***}&     -0.0165\sym{***}&     -0.0242\sym{***}\\
                    &     (-6.50)         &     (-9.98)         &     (-6.49)         &     (-9.98)         \\
Bid-Offer           &      0.0244\sym{***}&      0.0345\sym{***}&      0.0246\sym{***}&      0.0345\sym{***}\\
                    &     (10.38)         &     (14.70)         &     (10.31)         &     (14.70)         \\
Second Half Dummy   &      -0.382\sym{***}&      -0.316\sym{***}&      -0.381\sym{***}&      -0.316\sym{***}\\
                    &     (-8.64)         &     (-7.87)         &     (-8.62)         &     (-7.86)         \\
constant            &       0.178\sym{***}&       0.116\sym{***}&       0.177\sym{***}&       0.116\sym{***}\\
                    &      (6.86)         &      (5.03)         &      (6.73)         &      (5.02)         \\
\midrule
Round FE            &          NO         &          NO         &          NO         &          NO         \\
Simulation FE       &          NO         &         YES         &          NO         &         YES         \\
Market Type FE      &          NO         &          NO         &         YES         &         YES         \\
Adjusted R-Squared  &       0.257         &       0.338         &       0.260         &       0.338         \\
N                   &       3,211         &       3,211         &       3,211         &       3,211         \\
\bottomrule
\end{tabular*}
}


==> Tables/Table_expectation_trading_controls.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular*}{1.0\hsize}{@{\hskip\tabcolsep\extracolsep\fill}l*{8}{cc}}
\toprule
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}&\multicolumn{1}{c}{(7)}&\multicolumn{1}{c}{(8)}\\
                    &\multicolumn{8}{c}{}\\
\midrule
Expectation (t)     &      -0.209\sym{*}  &      -0.152         &                     &                     &                     &                     &                     &                     \\ % [SO: Fixed from "t to t+1"]
                    &     (-2.10)         &     (-1.62)         &                     &                     &                     &                     &                     &                     \\
Expectation (t+2)   &                     &                     &     -0.0442         &     -0.0443         &                     &                     &                     &                     \\ % [SO: Fixed from "t to t+2"]
                    &                     &                     &     (-0.78)         &     (-0.84)         &                     &                     &                     &                     \\
Expectation (t+5)   &                     &                     &                     &                     &      0.0218         &      0.0380         &                     &                     \\ % [SO: Fixed from "t to t+5" — was correct but relabeled for consistency]
                    &                     &                     &                     &                     &      (0.52)         &      (0.95)         &                     &                     \\
Expectation (t+10)  &                     &                     &                     &                     &                     &                     &      0.0645\sym{*}  &      0.0697\sym{*}  \\ % [SO: Fixed from "t to t+10" — was correct but relabeled for consistency]
                    &                     &                     &                     &                     &                     &                     &      (2.38)         &      (2.67)         \\
Recent Return (t-1 to t)&       0.475\sym{***}&       0.138         &       0.464\sym{***}&       0.134         &       0.430\sym{***}&      0.0938         &       0.397\sym{***}&      0.0771         \\
                    &      (6.33)         &      (1.91)         &      (6.33)         &      (1.79)         &      (6.24)         &      (1.31)         &      (5.98)         &      (1.12)         \\
Recent Return (t-2 to t-1)&       0.275\sym{***}&      0.0849         &       0.247\sym{**} &      0.0682         &       0.209\sym{**} &      0.0262         &       0.183\sym{*}  &      0.0160         \\
                    &      (4.05)         &      (1.22)         &      (3.55)         &      (0.94)         &      (3.08)         &      (0.36)         &      (2.71)         &      (0.23)         \\
Recent Return (t-3 to t-2)&       0.166\sym{*}  &      0.0406         &       0.144         &      0.0267         &       0.121         &     0.00378         &       0.112         &     0.00931         \\
                    &      (2.06)         &      (0.47)         &      (1.73)         &      (0.30)         &      (1.43)         &      (0.04)         &      (1.42)         &      (0.11)         \\
Recent Return (t-4 to t-3)&       0.243\sym{*}  &       0.125         &       0.231\sym{*}  &       0.116         &       0.220\sym{*}  &       0.109         &       0.223\sym{*}  &       0.124         \\
                    &      (2.40)         &      (1.11)         &      (2.28)         &      (1.05)         &      (2.19)         &      (1.01)         &      (2.34)         &      (1.19)         \\
\midrule
Investor FE         &         YES         &         YES         &         YES         &         YES         &         YES         &         YES         &         YES         &         YES         \\
Round FE            &          NO         &         YES         &          NO         &         YES         &          NO         &         YES         &          NO         &         YES         \\
Simulation FE       &          NO         &         YES         &          NO         &         YES         &          NO         &         YES         &          NO         &         YES         \\
Adjusted R-Squared  &       0.599         &       0.602         &       0.599         &       0.602         &       0.599         &       0.602         &       0.599         &       0.603         \\
N                   &      43,581         &      43,581         &      43,573         &      43,573         &      43,567         &      43,567         &      43,567         &      43,567         \\
\bottomrule
\end{tabular*}
}


==> Tables/Table_plan_insights.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular*}{1.0\hsize}{@{\hskip\tabcolsep\extracolsep\fill}l*{2}{cc}}
\toprule
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}\\
                    &\multicolumn{1}{c}{} &\multicolumn{1}{c}{} \\
\midrule
Stated Actions in Insights&       0.350\sym{***}&       0.333\sym{***}\\
                    &     (58.71)         &     (56.80)         \\
\midrule
Investor FE         &         YES         &         YES         \\
Round FE            &          NO         &         YES         \\
Simulation FE       &          NO         &         YES         \\
Adjusted R-Squared  &       0.421         &       0.425         \\
N                   &      68,739         &      68,739         \\
\bottomrule
\end{tabular*}
}

